A Practical Introduction to Side-Channel Extraction of Deep Neural Network Parameters

Model extraction is a major threat for embedded deep neural network models that leverages an extended attack surface. Indeed, by physically accessing a device, an adversary may exploit side-channel leakages to extract critical information of a model (i.e., its architecture or internal parameters). Different adversarial objectives are possible including a fidelity-based scenario where the architecture and parameters are precisely extracted (model cloning). We focus this work on software implementation of deep neural networks embedded in a high-end 32-bit microcontroller (Cortex-M7) and expose several challenges related to fidelity-based parameters extraction through side-channel analysis, from the basic multiplication operation to the feed-forward connection through the layers. To precisely extract the value of parameters represented in the single-precision floating point IEEE-754 standard, we propose an iterative process that is evaluated with both simulations and traces from a Cortex-M7 target. To our knowledge, this work is the first to target such an high-end 32-bit platform. Importantly, we raise and discuss the remaining challenges for the complete extraction of a deep neural network model, more particularly the critical case of biases.

==> figures/xtr_flowchart.tex <==
\begin{figure}[b]
	\centering
	\includegraphics[width=0.99\textwidth]{./figures/xtr_process_flowchart.pdf}
	\caption{Flowchart representing extraction process steps with their respective inputs, parameters and outputs.}
	\label{xtr_process_flowchart}
\end{figure}

